Bullshark: DAG BFT Protocols Made Practical

We present Bullshark, the first directed acyclic graph (DAG) based asynchronous Byzantine Atomic Broadcast protocol that is optimized for the common synchronous case. Like previous DAG-based BFT protocols, Bullshark requires no extra communication to achieve consensus on top of building the DAG. That is, parties can totally order the vertices of the DAG by interpreting their local view of the DAG edges. Unlike other asynchronous DAG-based protocols, Bullshark provides a practical low latency fast-path that exploits synchronous periods and deprecates the need for notoriously complex view-change mechanisms. Bullshark achieves this while maintaining all the desired properties of its predecessor DAG-Rider. Namely, it has optimal amortized communication complexity, it provides fairness and asynchronous liveness, and safety is guaranteed even under a quantum adversary. In order to show the practicality and simplicity of our approach, we also introduce a standalone partially synchronous version of Bullshark which we evaluate against the state of the art. The implemented protocol is embarrassingly simple (200 LOC on top of an existing DAG-based mempool implementation (Narwhal & Tusk). It is highly efficient, achieving for example, 125,000 transaction per second with a 2 seconds latency for a deployment of 50 parties. In the same setting the state of the art pays a steep 50% latency increase as it optimizes for asynchrony.

==> background.tex <==
\section{Background and Related Work}
\label{sec:relwork}
In~\secref{sec:intro} you talked about the project at a very high-level. This is
the section from where you will start giving details. First with things that are
already done, and familiarize the reader with background information they will
need to understand you work. 


\paragraph{Threat model.}
Often this section you will discuss the threat-model, but there is no strict consensus on that. 


Here is how you cite papers. For example, we read papers in the
class~\cite{rahul2016pwtypos,dodisetal:2004}.  And here is some random citation~\cite{Bojinov:2010:KLP,schechter:2010:pen,everspaugh2015pythia,bellare2009format,Juels:2014}


\subsection{Overview of the design}
\label{sec:overview}

And then just to showoff some \LaTeX skills, here is a Tikz plot.
\input{images/mainflow.tex}

You refer to a figure in the following way. In~\figref{fig:mainflow} we show
some thing that is relevant for the Multisketch paper by Chatterjee et
al.~\cite{chatterjee2019multisketches}. Add your bibliography to the
\textsf{bib.bib} file. You can copy the Bibtex format citation from Google
Scholar.


==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> proofs_partial_sync.tex <==
\section{Proofs}
\label{sec:proofs}

We provide proofs of correctness for both versions of \sys. 
%For space limitations, the proof of the eventually synchronous version is defer to Appendix~\ref{app:ESproof}.

\subsection{\sys With Fallback}
\label{sec:fallback}

\paragraph{Total order.}
%
Note that at any given time parties might have slightly different local DAGs.
This is because some vertices may be delivered at some parties but not yet at others.
However, since we use reliable broadcast for each vertex $v$, and wait for the entire causal history of $v$ to be added to the before we add $v$, we get the following important observation:

\begin{observation}
\label{obs:relaible}
For every two honest parties $p_i$ and $p_j$ we get:
\begin{itemize}
    \item For every round $r$, $\bigcup_{r > 0} DAG_i[r]$ is eventually equal to\\ $\bigcup_{r > 0} DAG_j[r]$.
    \item For any given time $t$ and round $r$, if $v \in DAG_i[r]$ $\wedge$  $v' \in DAG_i[r]$ s.t.\ $v.source = v'.source$, then $v = v'$.
    Moreover, for every round $r'<r$, if $v'' \in DAG_i[r']$ and there is a path from $v$ to $v''$, then $v'' \in DAG_j[r']$ and there is a path between $v'$ to $v''$. 
\end{itemize}
\end{observation}

To totally order the vertices in the DAG, each party $p_i$ locally interprets $DAG_i$ (there is no extra communication on top of building the DAG).
To this end, $p_i$ divides its DAG into waves of 4 rounds each. 
Every wave has 3 leaders that can potentially be committed: 2 steady-state leaders and one fallback leader.
The steady-state leaders are two pre-defined vertices, one in the first round of the wave and the other in the third.
The fallback leader is a vertex in the first round of the wave that is selected by the randomness produced in the fourth round of the wave. 
%Below we show that a steady-state leader and a fallback leader cannot be committed in the same wave.
To make sure a fallback leader and a steady state leader are not committed in the same wave, each party can only vote for either the fallback leader or the steady-state ones.
In the code, \emph{steadyVoters[w]} \emph{fallbackVoters[w]} contain all the parties that can vote for steady-state or fallback leaders in wave $w$, respectively.
We say that a party $p_i$ \emph{determines} $p_j$ \emph{vote type} to be a steady-state (fallback)  in wave $w$ if its $\emph{steadyVoters}[w]$ ($fallbackVoters[w]$) contains $p_j$. 
Moreover, as we show in the next claim, all parties agree on $p_j$'s vote type in wave $w$.
This, in particular, means that Byzantine parties cannot equivocate or hide their vote (a nice property that we get from using reliable broadcast as a building block). 
%
\begin{claim}
\label{claim:votetype}

For every party $p_i$ and round $r$, each party $p_j$ determines at most one vote type for $p_i$ in wave $w$.
Moreover if $p_j$ and $p_k$ determine vote type $T$ and $T'$ for $p_i$ in wave $w$, respectively, then $T = T'$.  

\end{claim}
%
\begin{proof}
The first part of the claim follows from the code of function $\emph{determine\_party\_vote\_type}$.
This function is called by a party $p_j$ whenever it adds a new vertex $v$ to $DAG_j[r]$ such that $r$ is the first round of a wave, and the source of the vertex (a party $p_i$) is either added to \emph{steadyVoters[w]} or \emph{fallbackVoters[w]}.
The second part of the claim follows from Observation~\ref{obs:relaible} and the fact (by the code of try\_add\_to\_DAG) that $v$ is added to the DAG only after all its causal history is added.
This guarantees that for every wave $w$ and party $p_i$ try\_steady\_commit and try\_fallback\_commit are called with the same parameters and thus return the same result.
This in turn guarantees that all parities that determine $p_i$'s vote type in wave $w$ see the same type. %\qedsymbol{}
%
\end{proof}

\vspace{2mm}
There are two possible ways to commit a leader $v$ in \sys.
The first is to \emph{directly} commit it when either try\_steady\_commit or try\_fallback\_commit, called with $v$, return true.
The second option is to \emph{indirectly} commit it when it is added to \emph{leaderStack} in Line~\ref{line:stacksteady} or~\ref{line:stackfallback}.
In both cases, to commit a leader in wave $w$, we count the number of vertices in some round (depending on the leader type and whether we directly or indirectly commit it) in $w$ that have a strong path to the leader and their vote corresponds to the leader's type. 
%\neil{Not necessarily $r+1$ since the fallback leader you look at round $r+3$. Maybe rephrase to say that if a leader is committed in round $r$ we count the number of vertices in $r$ that have a strong path to the leader.}
%\sasha{resolved. "in round $r$" is confusing as one can think the leader is in round $r$.}. 
We first show that steady state and fallback leaders cannot be directly committed in the same wave.

\begin{claim}
\label{claim:samewave}

If a party $p_i$ directly commits a steady-state leader in wave $w$, then no party commits (directly or indirectly) a fallback leader in wave $w$, and vice versa.

\end{claim}

\begin{proof}
%
Consider a steady state leader vertex $v$ committed by a party $p_i$ in round $r$ in wave $w$.
By the code, to directly commit a leader vertex a party need to determine the vote type of at least $2f+1$ parties in the wave to be the same as the leaders.
Similarly, to indirectly commit a vertex leader, a party needs to determine the vote type of at least $f+1$ parties in the wave to be the same as the leaders.
Since $p_i$ directly commits state leader vertex $v$ in wave $w$, it determines $2f+1$ parties as steady state voters in wave $w$.
Since there are $3f+1$ parties in total, by Claim~\ref{claim:votetype}, no other party determines more than $f$ parties as fallback voters in wave $w$.
Therefore, no other party commit (directly or indirectly) a fallback leader in wave $w$.
From symmetry, the same argument works in the other direction.
%
\end{proof}

\vspace{2mm}
For the proof of the next lemmas we say that a party $p_i$ \emph{consecutively directly commit} leader vertices $v_i$ and $v'_i$ if $p_i$ directly commits them in rounds $r_i$ and $r'_i > r_i$, respectively, and does not directly commit any leader vertex between $r_i$ and $r'_i$. 
In the next claims we are going to show that honest parties commit the same leaders and in the same order:

\begin{claim}
\label{claim:commitmin}

Let $v_i$ and $v'_i$ be two leader vertices consecutively directly committed by a party $p_i$ in rounds $r_i$ and $r'_i > r_i$, respectively.
Let $v_j$ and $v'_j$ be two leader vertices consecutively directly committed by a party $p_j$ in rounds $r_j$ and $r'_j > r_j$, respectively.
If $r_i \leq r_j \leq r'_i$, then both $p_i$ and $p_j$ (directly or indirectly) commit the same leader in round $min(r'_i,r'_j)$.

\end{claim}

\begin{proof}
%
Claim~\ref{claim:samewave} implies that that there is at most one committed leader in each round.
Thus, if $r'_i = r'_j$ we are done.
Otherwise, assume without lost of generality that $r'_i < r'_j$.
Thus, if $r_j = r'_i$ we are done.
Otherwise, we need to show that $p_j$ indirectly commits $v'_i$ in $r'_i$.

By the code of commit\_leader, after $p_j$ directly commits $v_j'$ in round $r'_j$ it tries to indirectly commit leaders in round numbers smaller than $r'$ until it reaches round $r_j < r'_i$.
Let $r'_i < r < r'_j$, be the smallest number between $r'_i$ and $r'_j$ in which $p_j$ (directly or indirectly) commits a leader $v$.
Consider two cases:
\begin{itemize}
    \item Vertex $v'_i$ is a steady-state leader.
    Note that $r > r'_i + 1$ since only odd rounds have potential leaders.
    Since $p_i$ directly commits $v'_i$ in round $r'_i$, there is a set $C$ of $2f+1$ vertices in $DAG_i[r'_i + 1]$ with strong paths to $v'_i$ and with $v'_i$'s types. By observation~\ref{obs:relaible}, Claim~\ref{claim:votetype}, and quorum intersection, there are at least $f+1$ vertices in $DAG_j[r'_i + 1]$ with $v'_i$'s vote type and strong paths from the $v$ to them.
    
    \item Vertex $v'_i$ is a fallback leader. 
    By Claim~\ref{claim:samewave}, no leader is committed in round $r+2$.
    Thus, $r > r'_i + 3$.
    Since $p_i$ directly commits $v'_i$ in round $r'_i$ and $v_i$, there is a set $C$ of $2f+1$ vertices in $DAG_i[r'_1 + 3]$ with strong paths to $v'_i$ and with $v'_i$'s types. 
    By observation~\ref{obs:relaible}, Claim~\ref{claim:votetype}, and quorum intersection, there are at least $f+1$ vertices in $DAG_j[r'_i + 3]$ with $v'_i$'s vote type and strong paths from the $v$ to them.
\end{itemize}
%
I both cases $p_j$ counts (in \emph{ssVotes} or \emph{fbVotes}) at least $f+1$ votes for the leader.
In addition, by observation~\ref{obs:relaible} and Claim~\ref{claim:votetype}, since in both cases there are at least $2f+1$ vertices with the $v$'s type, there are at most $f$ vertices with the opposite type. 
Thus, $p_j$ counts at most $f$ votes for the other leader.
Therefore, by Lines\ref{line:indirectfirst}-\ref{line:indirectlast} in commit\_leader, $p_j$ indirectly commits $v'_i$.


%Note that $r > r'_i + 1$ since only odd rounds have potential leaders.
%Since $p_i$ directly commits $v'_i$ in round $r'_i$, 
%there is a set $C$ of $2f+1$ vertices in $DAG_i[r'_i + 1]$\neil{or $DAG_i[r'_1 + 3]$} with strong paths to $v'_i$ and with $v'_i$'s types (fallback or steady-state).
%By observation~\ref{obs:relaible}, Claim~\ref{claim:votetype}, and quorum intersection, there are at least $f+1$ vertices in $DAG_j[r'_i + 1]$ \neil{or $DAG_i[r'_1 + 3]$} with $v'_i$'s vote type and strong paths from the $v$ to them.
%In addition, by observation~\ref{obs:relaible} and Claim~\ref{claim:votetype}, there are at most $f$ vertices in $DAG_j[r'_i + 1]$ with $v'_i$'s vote type and strong paths from the $v$ to to them.
%Therefore, by the code of commit\_leader, $p_j$ indirectly commits $v'_i$.

\end{proof}

\begin{claim}
\label{claim:commitinterval}

Let $v_i$ and $v'_i$ be two leader vertices consecutively directly committed by a party $p_i$ in rounds $r_i$ and $r'_i > r_i$, respectively.
Let $v_j$ and $v'_j$ be two leader vertices consecutively directly committed by a party $p_j$ in rounds $r_j$ and $r'_j > r_j$, respectively.
Then $p_i$ and $p_j$ commits the same leaders between rounds $max(r_i,r_j)$ and $min(r'_i,r'_j)$, and in the same order.

\end{claim}

\begin{proof}
%
If $r'_i < r_j$ or $r'_j < r_i$, then we are trivially done because there are no rounds between $max(r_i,r_j)$ and $min(r'_i,r'_j)$.
Otherwise, assume without lost of generality that $r_i \leq r_j \leq r'_i$.
By Claim~\ref{claim:commitmin}, both $p_i$ and $p_j$ (directly or indirectly) commit the same leader in round $min(r'_i,r'_j)$.
Assume without lost of generality that $min(r'_i,r'_j) = r'_i$.
Thus, by Claim~\ref{claim:samewave}, both $p_i$ and $p_j$ commit $v'_i$ in round $r'_i$ and $v_j$ in round $r_j$.
By the code of commit\_leader, after (directly or indirectly) committing a leader, parties try to indirectly commit leaders in smaller round numbers until they reach a round in which they previously directly committed a leader.
%\sasha{I skip here some details. Maybe I will do anther pass and add them. Here comes the recursive way in which we go back.}
Therefore both $p_i$ and $p_j$ will try to indirectly commit all leaders going down from $r'_i = min(r'_i,r'_j)$ to $r_j = max(r_i,r_j)$.
Since $v'_i$ appears in both $DAG_i$ and $DAG_j$, by Observation~\ref{obs:relaible}, all vertices in $DAG_i$ such that there is a path from $v'_i$ to them appear also in $DAG_j$.
The claim follows from the deterministic code of the function commit\_leader.

\end{proof}

\vspace{2mm}
By inductively applying Claim~\ref{claim:commitinterval} for every pair of honest parties  we get the following:

\begin{corollary}
\label{col:order}

Honest parties commit the same leaders and in the same order.

\end{corollary}

For the next lemma we say that the \emph{causal history} of a vertex leader $v$ in the DAG is the set of all vertices such that there is a path from $v$ to them.

\begin{lemma}
\label{lem:order}

Algorithms~\ref{alg:dataStructures}, \ref{alg:DAG}, \ref{alg:modes}, and~\ref{alg:commit} satisfy Total order.

\end{lemma}

\begin{proof}
%
By Corollary~\ref{col:order}, honest parties commit the same leaders and in the same order.
By the code of the order\_vertices procedure, parties iterate on the committed leaders according to their order and  \emph{a\_deliver} all vertices in their causal history by a pre-defined deterministic rule.
The lemma follows by Observation~\ref{obs:relaible} since all honest parties has the same casual history in their DAG for every committed leader.

\end{proof}

\paragraph{Agreement and Validity.}

\begin{lemma}
\label{lem:agreement}

Algorithms~\ref{alg:dataStructures}, \ref{alg:DAG}, \ref{alg:modes}, and~\ref{alg:commit} satisfy Agreement.

\end{lemma}

\begin{proof}
%
Assume some honest party $p_i$ outputs $a\_deliver(v_i.block,\\ v_i.round, v_i.source)$.
We will show that every honest party $p_j$ outputs it as well.
By the code of order\_vertices, there is a leader vertex $v$ that $p_i$ committed such that $v_i$ is in $v$'s casual history.
By Observation~\ref{obs:relaible}, the $v$'s casual histories in $DAG_i$ and $DAG_j$ are the same.  
Thus, by code of order\_vertices, we only need to show that $p_j$ eventually commit leader vertex $v$.
Let $v'$ be the leader vertex with the lowest number that is higher than $v.round$ that $p_i$ directly commits.
Let $v''$ be the vertex that triggers this direct commit, i.e., the vertex $v''$ that passed to the try\_ordering function that calls determine\_party\_vote\_type, which in turn commits $v'$.
By Observation~\ref{obs:relaible}, $p_j$ eventually add $v''$ to $DAG_j$ and call try\_ordering with $v''$.
By Observation~\ref{obs:relaible} again, the casual history of $v''$ in $DAG_i$ is equivalent the casual history of $v''$ in $DAG_j$.
Hence, $p_j$ directly commits $v'$ as well.
Since the casual history of $v'$ in $DAG_i$ is also equivalent the casual history of $v'$ in $DAG_j$, $p_j$ also commits $v$.

\end{proof}

\vspace{2mm}
By the Liveness (Agreement and Validity) properties of reliable broadcast and since it is enough for parties to deliver $2f+1$ vertices in a round in order to move to the next one, the DAG grows indefinitely:

\begin{observation}
\label{obs:DAGgrows}

For every round $r$ and honest party $p_i$, $DAG_i[r]$ eventually contains a vertex for every honest party.

\end{observation}


In the next to claims we show that for every round $r$ there is an honest party $p_i$ that commit a leader in a round higher than $r$ with probability $1$. First, we show that if it is not the case, then starting from some point the vote type of all parties is fallback. Note that this is true also for Byzantine parties since thanks to the reliable broadcast Byzantine parties cannot lie about their casual history.

\begin{claim}
\label{claim:honestfallback}

Consider an honest party $p_i$.
If there is a wave $w$ after which no honest party commits a leader, then in all waves $w' >w +1$ $p_i$ determines the vote type of all parties that reach $w'$ in $DAG_i$ as fallback. 

\end{claim}

\begin{proof}
%
Let $w' > w + 1$ be a wave that start after $w$. By the claim assumption no honest party commits a leader in wave $w' -1$. Let $r$ be the first round of wave $w'$. 
%By Observation~\ref{obs:DAGgrow}, $DAG_i[r]$ eventually contains a vertex for every honest party $p_j$.
Consider a party $p_j$ for which $p_i$ has a vertex $v_j$ in $DAG_i[r]$
By the code, $p_i$ calls try\_ordering with $v_j$, which in turn calls determine\_party\_vote\_type to determine $p_j$'s vote type for $w'$.
By Observation~\ref{obs:relaible}, the casual history of $v_j$ in $DAG_j$ is equivalent to the casual history of $v_j$ in $DAG_i$.
The claim follows from the code of determine\_party\_vote\_type.
Since $p_j$ did not commit a leader in wave $w'$, both functions try\_steady\_commit and try\_fallback\_commit return falls $p_i$' invocation of\\ determine\_party\_vote\_type.
Therefore, $p_i$ sets $p_j$'s vote type in $w'$ to fallback.

\end{proof}

\vspace{2mm}
The following claim is a known property of all to all communication, which sometimes referred as \emph{common core}~\cite{canetti1996studies}.
We provide proof for completeness.

\begin{claim}
\label{claim:core}

For every wave $w$ and party $p_i$.
Let $r$ be the first round of $w$.
If $|DAG_i[r+k]| \geq 2f+1, k \in \{0,1,2,3\}$, then there is a set $C \subseteq DAG_i[r]$ such that $|C| = 2f+1$ and for every vertex $v \in C$ there are $2f+1$ vertices in $DAG_i[r+3]$ with strong paths to $v$.

\end{claim}

\begin{proof}
%
The proof follows from the fact that every vertex in every round of the DAG has at least $2f+1$ strong edges to vertices in the previous round.
In particular, it is easy to show by a counting argument that there is one vertex $u \in DAG_i[r_1]$ such that $f+1$ vertices in $DAG_i[r+2]$ has a strong edge to $u$.
Therefore, by quorum intersection, every vertex in $DAG_i[r+3]$ has a strong path to $u$.
Let $C \subseteq DAG_i[r]$, $|C| = 2f+1$ be the set of vertices that $u$ has a strong path to, then every vertex in $DAG_i[r+3]$ has a strong path to every vertex in $C$.
The lemma follows since there are at least $2f+1$ vertices in $DAG_i[r+3]$.

\end{proof}

\vspace{2mm}
Next, we use the fact that fallback leaders are hidden from adversary until the last round of a wave to prove the following: 


\begin{claim}
\label{claim:probcommit}

Consider a party $p_i$ and a wave $w$ such that $p_i$ determines the vote type of all parties that reach $w$ in $DAG_i$ as fallback.
Then the probability of $p_i$ to commit the fallback vertex leader of $w$ is at least $2/3$.

\end{claim}

\begin{proof}
%
Let $r$ be the first round of $w$.
By the assumption, the vote type of all parties with vertices in $DAG_i[r+3]$ is fallback.
Therefore, by Claim~\ref{claim:core}, there are at least $2f+1$ vertices in the first round of $w$ that satisfy the fallback  commit rule.
That is, there is a set $C$ of $2f+1$ parties such that if any of them is elected to be the fallback leader, then $p_i$ will commit it.
Since the fallback leader is elected with the randomness produced in round $r+3$, the set $C$ is determined before the adversary learns the leader.
Therefore, even though the adversary fully controls delivery times, the probability for the elected leader to be in $C$ is at least $2f+1/3f+1 > 2/3$.

\end{proof}

\vspace{2mm}

\begin{claim}
\label{claim:somecommit}
For every wave $w$, there is an honest party that with probability $1$ commits a leader in a wave higher than $w$.
\end{claim}

\begin{proof}
%
Assume by a way of contradiction no honest party commits a leader in a wave higher than $w$.
By Observation~\ref{obs:DAGgrows}, for every round $r$ and honest party $p_i$, $DAG_i[r]$ eventually contains at least $2f+1$ vertices.
Moreover, by Claim~\ref{claim:honestfallback}, there is an honest party $p_i$ that determines the vote type of all parties that reach $w' > w +1$ in $DAG_i$ as fallback.
Therefore, by Claim~\ref{claim:probcommit}, the probability of $p_i$ to
commit the fallback leader in any wave $w' > w+1$ is at least $\frac{2}{3}$.
Hence, with probability $1$, there is a wave higher than $w$ that $p_i$ commits.

\end{proof}

%\vspace{2mm}
%The intuition for the Liveness of DAG-Riders is the following:
%By applying a combinatorial argument it is easy to show that there is a set $C$ of at least $2f+1$ vertices in the first round of each wave such that for vertex $v \in C$, there are $2f+1$ vertices in the forth round of the wave with strong paths to $v$.
%Therefore, if the fallback leader of the wave is elected to be one of the vertices in the set $C$, then the commit rule is satisfied since the vote type of all parties is fallback.
%Since the fallback leader is elected only after the set $C$ is determined, each wave is committed with probability $2/3$.
%The full proof can be found in~\cite{keidar2021all}.

\vspace{2mm}
We next use Claim~\ref{claim:somecommit} to prove Validity.

\begin{lemma}
\label{lem:validity}

Algorithms~\ref{alg:dataStructures}, \ref{alg:DAG}, \ref{alg:modes}, and~\ref{alg:commit} satisfy Validity.

\end{lemma}

\begin{proof}
%
Let $p_i$ be an honest party that calls $a\_bcast(b,r)$, we need to show that all honest parties output $a\_deliver(b,r,p_i)$ with probability $1$.
By the code $p_i$ pushes $b$ in the \emph{blockToPropose} queue.
By Observation~\ref{obs:DAGgrows}, $p_i$ advanced unbounded number of rounds and thus creates unbounded number of vertices.
Therefore, eventually $p_i$ will create a vertex $v_i$ with $b$ and reliably broadcast it.
By the Validity property of reliably broadcast, all honest parties will eventually add it to their DAG. 
That is, for every honest party $p_j$, there is a round number $r_i$ such that $v_i \in DAG_j[r_i]$. 
By the code of create\_new\_vertex, every vertex that $p_j$ creates after $v_i$ is added to $DAG_j[r_i]$ have a path to $v_i$ (either with strong links or weak links).
%By Observation~\ref{obs:DAGgrows}, there is such vertex and lets denote it by $v$.

Therefor, by Claim~\ref{claim:somecommit}, there is an honest party $p_j$ that with probability $1$ commits a leader vertex with a path to $v_i$. 
Thus, by the code of order\_vertices, $p_i$ outputs $a\_deliver(b,r,p_i)$ with probability $1$.
Since $p_i$ is honest, we get that by Lemma~\ref{lem:agreement} (Agreement), all honest parties output $a\_deliver(b,r,p_i)$ with probability $1$.

\end{proof}

\paragraph{Integrity.}
\begin{lemma}
\label{lem:integrity}
Algorithms~\ref{alg:dataStructures}, \ref{alg:DAG}, \ref{alg:modes}, and~\ref{alg:commit} satisfy Integrity.
\end{lemma}

\begin{proof}
An honest party $p_i$ outputs $a\_deliver(v'.block,v'.round,\\ v'.source)$ only if node $v'$ is in $p_i$'s DAG (i.e., $v' \in \bigcup_{r > 0} DAG_i[r]$).
Node $v'$ is added to $p_i$'s DAG upon the reliable broadcast\\ $r\_deliver(v',v'.round, v'.source)$ event.
Therefore, the Lemma follows from the Integrity property of reliable broadcast.  
\end{proof}



\subsection{Partially Synchronous \sys}
\label{sub:ESproof}

The proof of the Integrity property is identical to the proof of Lemma~\ref{lem:integrity}.
For the rest of the properties, due to similarities between the protocols and to avoid argument duplication, we will follow the structure of Section~\ref{sec:fallback} and sometimes explain how to adapt claims' proofs.

To be consistent with the \sys with fallback presentation, waves here are also consist of 4 rounds, each with a pre-defined leader in the first and fourth rounds (we could have waves of 2 rounds since we do not have the fallback leader).

\paragraph{Total order.}
Observation~\ref{obs:relaible} applies in this case as well because the protocol to build the DAG is the same.
Claim~\ref{claim:votetype} trivially holds here since there is only one possible vote type and Claim~\ref{claim:samewave} holds since there are no fallback leaders.
The proofs of Claims~\ref{claim:commitmin} and~\ref{claim:commitinterval} apply to Algorithm~\ref{alg:ESBullshark} as well.
Therefore, Corollary~\ref{col:order} applies and since we use the same order\_vertices procedure in both protocols we get:

\begin{lemma}
\label{lem:ESorder}

Algorithms~\ref{alg:dataStructures}, \ref{alg:DAG}, \ref{alg:modes}, and~\ref{alg:ESBullshark} satisfy Total order.

\end{lemma}

\paragraph{Agreement and Validity.}

The proof of the Agreement property is identical to the proof of Lemma~\ref{lem:agreement} and Observation~\ref{obs:DAGgrows} holds since the algorithm to build the DAG is the same as in \sys with fallback.
To proof Validity for the eventually synchronous variant of \sys we do not need Claims~\ref{claim:honestfallback} and~\ref{claim:somecommit}.
Instead, we use the fact that GST eventually occurs.
%For the next claim we assume that after GST each reliable broadcast (from honest broadcast to all honest deliveries) takes $\Delta$ time and the timeouts (Line~\ref{line:time}) are set for $2\Delta$. \sasha{revisit}
We prove the protocol under the assumption that honest parties set their timeouts to be larger than $3\Delta$ and the following holds for the reliable broadcast building block:

\begin{property}
\label{prop:relaible}

Let $t$ be a time after GST. 
If an honest party reliably broadcasts a message at time $t$ or an honest party delivers a message at time $t$ , then all honest parties deliver it by time $t + \Delta$.

\end{property}

The above property is the equivalent to the reliable broadcast Validity and Agreement properties in the asynchronous model.
To the best of our knowledge, it is satisfied by all reliable broadcast protocol since before delivering a message honest parties echo it to all other honest parties.
%The following claim follows directly from Property~\ref{prop:relaible}:



\begin{claim}
\label{claim:EScommit}

Let $w$ be a wave such that all honest parties advances to the first round of $w$ after GST.
Let $p_1$ and $p_2$ be their first and second pre-defined leaders of $w$, respectively.
If $p_1$ and $p_2$ are honest, then all honest parties commit a leader in $w$.

\end{claim}

\begin{proof}
%
let $r$ be the first round of $w$.
First we show that all honest parties advance to round $r+1$ within $2\Delta$ time of each other.
By Observation~\ref{obs:DAGgrows}, all honest parties eventually advance to round $r+1$.
Let party $p_i$ be the first honest party that advances to round $r+1$ and denote by $t$ the time it happened. 
By the code of try\_advance\_round, $|DAG_i[r]| \geq 2f+1$.
By Property~\ref{prop:relaible}, by time $t + \Delta$ $|DAG_j[r]| \geq 2f+1$ for all honest parties.
Therefore, by Line~\ref{line:time2}, all honest party advance to round $r$ by time $t + \Delta$.
In particular, the first leader of wave $w$, $p_1$.
Thus, $p_1$ broadcasts its vertex $v_1$ in round $r$ no later than time $t + \Delta$, and by Property~\ref{prop:relaible}, all honest deliver it by time $t + 2\Delta$.
Therefore, by Line~\ref{line:advance1} and the code of try\_advance\_round, all honest parties advance to round $r+2$ by time $t + 2\Delta$.

Next we show that all honest parties advance to round $r+2$ with $3\Delta$ time of each other.
Since all honest parties advance to round $r+1$ within $2\Delta$ time of each other, then they start their timeouts at round $r+1$ within $2\Delta$ time of each other.
Let party $p_j$ be the first honest party that advances to round $r+2$.
If the first honest party waits for timeout (the if in Line~\ref{line:advance2}) to advance to round $r+2$, then all honest parties advance to round $r+2$ within $2\Delta$.
Otherwise, $p_j$ has $2f+1$ vertices in $DAG_j[r+1]$ with strong path to $v'$.
By property~\ref{prop:relaible}, all other honest parties will deliver this vertices and advance to round $r+2$ within $3\Delta$ from $p_j$.

By the assumption, the second leader of the wave, $p_2$, is honest and will broadcast vertex $v_2$ in round $r+2$ at most $3\Delta$ after the first honest party advances to $r+2$.
Since the timeouts are larger than $4\Delta$, all honest will advance to round $r+3$ within $\Delta$ of each other (by Line~\ref{line:advance3}, all honest wait to deliver the leader's vertex or for a timeout).
Moreover, they will all add a strong edge to $v_2$ in their vertex in round $r+3$.

Since all honest advance to round $r+3$ within $\Delta$ of each other and the timeouts are larger than $2\Delta$, they will all wait for each other's vertices before advancing to the next round.
Therefore, all honest will get $2f+1$ vertices in round $r+3$ with strong paths to the second vertex leader of the wave $v_2$.
Thus, all honest commit a leader in wave $w$. 

\end{proof}

\vspace{2mm}
The Validity property is proved under the assumption that eventually (after GST) there will be a wave in which both leaders are honest. For example, this assumption holds for every full permutation of the parties or if we maintain a fixed leader for the full wave.
To avoid repetition, we omit the proof of the following lemma as it is similar to the proof of Lemma~\ref{lem:validity}.
All we need to do to adapt it is to remove all appearances of "with probability $1$" and replace the reference to Claim~\ref{claim:somecommit} with Claim~\ref{claim:EScommit}.


\begin{lemma}
\label{lem:ECvalidity}

Algorithms~\ref{alg:dataStructures}, \ref{alg:DAG}, \ref{alg:modes}, and~\ref{alg:ESBullshark} satisfy Validity.

\end{lemma}




==> revise_proofs.tex <==
\section{Proofs Outline}

\begin{enumerate}
    \item Overview
    \item Steady state waves every 2 rounds, and fallback waves every 4 rounds
    \item The last round of a steady state or fallback wave is the round in which vertices are counted to determine the number of votes for a steady state or fallback
    leader. We also refer to this round as the \textit{voting round}.
    \item The last/voting round for a steady state wave w is round 2w, and the last/voting 
    round for a fallback wave w' is round 4w'
    \item Two waves conflict if they share the same last/voting round, for example steady state
    wave 2 conflicts with fallback wave 1, since they both share last/voting round 4 (2*2 = 4)
    \item In general an even steady state wave $w$ conflicts with fallback wave $w/2$
    \item Waves are ordered by their last/voting rounds. For example steady state wave 3 is less
    than fallback wave 2 since steady state wave 3 has voting round 2(3) = 6 and fallback
    wave 2 has voting round 4(2) = 8. Note that if two waves have the same voting round,
    they conflict. For example steady state wave 4 and fallback wave 2 have the same last 
    round.
    \item Once a validator enters a steady state or fallback wave it stays in that wave
    until the wave finishes (every 2 rounds or every 4 rounds respectively)
    \item A validator cannot be in two conflicting waves, for example a validator cannot be
    in both steady state wave 2 and fallback wave 1, or steady state wave 4 and fallback
    wave 2
    
\end{enumerate}

\begin{enumerate}
    \item Bullshark-Async: Total Order
    \item Lemma 1: If a correct validator commits a vertex $v$ in steady state wave $w$ then
    no other correct validator commits a vertex $v' \neq v$ in a conflicting fallback wave
    $w/2$
    \item Proof: Quorum intersection in the voting round $2w$.
    \item Lemma 2: If a correct validator commits a vertex $v$ in fallback wave $w$ then
    no other correct validator commits a vertex $v' \neq v$ in a conflicting steady state 
    wave $2w$
    \item Proof: Quorum intersection in the voting round $2w$.
    \item Lemma 3: If a correct validator commits a vertex $v$ in steady state wave $w$, then eventually all correct validators will commit $v$
    \item Proof: When a validator commits earlier leaders by quorum intersection it will see
    $f+1$ votes for $v$ and at most $f$ for the fallback leader
    \item Lemma 4: If a correct validator commits a vertex $v$ in fallback wave $w$, then eventually all correct validators will commit $v$
    \item Proof: When a validator commits earlier leaders by quorum intersection it will see
    $f+1$ votes for $v$ and at most $f$ for the steady state leader
    \item Lemma 5: If a correct validator orders vertex $v_1$ in wave $w_1$ before vertex
    $v_2$ in wave $w_2$, then $w_1 < w_2$
    \item Proof: Vertices are pushed onto the stack in decreasing wave order, and thus
    committed by increasing wave number
    \item Lemmas 1 and 2 ensure that correct validators commit at most 1 vertex in conflicting waves. Lemmas 3 and 4 ensure that validators commit the same vertices. Lemma
    5 ensures the correct validators commit vertices in the same order, namely by wave
    ordering. This satisfies total order since correct validators commit the same vertices
    and do so in the same order
\end{enumerate}

\begin{enumerate}
    \item Bullshark-Psync: Safety
    \item Lemma 1: If a correct validator commits vertex $v$ in steady state wave $w$ then
    every correct validator eventually also commits $v$
    \item Proof: When a validator goes to commit earlier leaders by quorum intersection there will exist at least 1 strong path
    \item Lemma 2: If a correct validator orders vertex $v_1$ in wave $w_1$ before vertex
    $v_2$ in wave $w_2$, then $w_1 < w_2$
    \item Proof: Vertices are pushed onto the stack in decreasing wave order, and thus are
    committed by increasing wave number
    \item Lemma 1 ensures correct validators commit the same vertices, and lemma 2 ensures
    they do so in the same order, satisfying safety
\end{enumerate}

\begin{enumerate}
    \item Bullshark-Psync: Liveness
    \item Lemma 1: After GST, if the leader of steady state wave $w$ is correct, then
    all correct validators will commit the steady state leader vertex of $w$.
    \item Proof: Every correct validator will begin the round within Delta, and receive the
    leader vertex within 2 Delta, since that is the time needed for reliable broadcast. Thus
    after 3 Delta all correct validators will add a strong edge to the leader vertex, since
    it is within the timeout. In the next round a correct validator again waits 3 Delta for
    all correct validators to enter the round and reliably broadcast their vertices, and
    thus it is guaranteed that all correct validators will see $2f+1$ votes for the steady
    state leader vertex and thus commit.
\end{enumerate}

\begin{enumerate}
    \item Communication Complexity
    \item For both Bullshark-Async and Bullshark-Psync, in each round every validator reliably broadcasts a vertex to be added into the
    DAG, so the communication complexity depends on which reliable broadcast protocol is
    used. To achieve the optimal communication complexity can use Cachin and Tessaro's AVID
    and batching to get an amortized O(n) communication complexity.
\end{enumerate}

\begin{enumerate}
    \item Round Complexity
    \item From the agreement property of Bullshark Async it takes an expected constant number of rounds to commit
    \item After GST with an honest leader, Bullshark Psync commits in 2 rounds from the
    liveness proof
\end{enumerate}
